Cooperative Aerial Robot Inspection Challenge: A Benchmark for Heterogeneous Multi-UAV Planning and Lessons Learned

We propose the Cooperative Aerial Robot Inspection Challenge (CARIC), a simulation-based benchmark for motion planning algorithms in heterogeneous multi-UAV systems. CARIC features UAV teams with complementary sensors, realistic constraints, and evaluation metrics prioritizing inspection quality and efficiency. It offers a ready-to-use perception-control software stack and diverse scenarios to support the development and evaluation of task allocation and motion planning algorithms. Competitions using CARIC were held at IEEE CDC 2023 and the IROS 2024 Workshop on Multi-Robot Perception and Navigation, attracting innovative solutions from research teams worldwide. This paper examines the top three teams from CDC 2023, analyzing their exploration, inspection, and task allocation strategies while drawing insights into their performance across scenarios. The results highlight the task's complexity and suggest promising directions for future research in cooperative multi-UAV systems.

==> preamble.tex <==

\usepackage[utf8]{inputenc}

%For page numbering
\pagenumbering{arabic}

% For lower case mathbb-like letters
\usepackage{mathbbol}

% For arrow on top of vector
\usepackage{esvect}

%For overlaying maths on the figure
\usepackage[percent]{overpic}

%For alignment in table
\usepackage{tabu}

% For multicolum
\usepackage{multicol}

% For multiple row in the table
\usepackage{multirow}
\def\mr{\multirow}
\def\mc{\multicolumn}

% For big bracket in composite equations
\usepackage[overload]{empheq}

% For bold font of greek letters
\usepackage{bm}

%For custom color schemes
\usepackage{xcolor}
\definecolor{dg}{rgb}{0.1, 0.6, 0.2}       %dg for dark green
\definecolor{b}{rgb}{0.0, 0.0, 1}          %b for basic blue

\usepackage{epsfig}
\usepackage{float}
\usepackage{color}
\usepackage{url}

% \usepackage{algorithm}      %for algorithm
% \usepackage[noend]{algpseudocode}
% \usepackage{algorithmic}
% \usepackage[ruled,linesnumbered,vlined]{algorithm2e}

% \usepackage[amssymb]{SIunits}
%\usepackage{amssymb, amsfonts, bbold}
\usepackage{amssymb, amsfonts}
\usepackage{amsmath}
\usepackage{mathrsfs}

\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{mathtools}

% \usepackage{bm}             %bold maths symbol

\let\labelindent\relax
% \usepackage{enumitem}       % for numbered items
% \setenumerate[enumerate]{align=left}

\usepackage{graphicx}
% \usepackage{subcaption}
% \usepackage{caption}
% \usepackage{subfigure}

% For better rumbering of reference
\usepackage{cite}

% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage{footmisc}   % For multiple references to the same footnote

% For overbraces in matrices
\usepackage{stackengine}

% To have table with notes at the bottom
\usepackage[flushleft]{threeparttable}

% Balancing the references at the end
% \usepackage{balance}

% To add appendix with title
% \usepackage[title]{appendix}


\newcommand{\ceil}[1]{\left\lceil   #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\Lim}[1]{\raisebox{0.5ex}{\scalebox{0.8}{$\displaystyle \lim_{#1}\;$}}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\obar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\renewcommand{\qedsymbol}{$\blacksquare$}   % To change qed symbol to square black box
\newcommand{\bref}[1]{(\ref{#1})}
\newcommand{\Mint}{%
  \mathrlap{\mathop{\phantom{\int}}\limits_{\!\mathbb{Q}}}%
  \!\int
}

\makeatletter
\newlength\tmp@\newlength\t@mp
\newcommand{\comp}[3]
  {\mathop{ \settowidth\tmp@{$\displaystyle\mathop{#1}^{#3}_{#2}$}
  \hbox to \tmp@{\hss \settowidth\t@mp{$\displaystyle #1$}\setlength\t@mp{.45\t@mp}
  $\displaystyle\mathop{#1}^{\hspace\t@mp #3}_{\hspace{-\t@mp}#2}$
  \hss} }}
\makeatother

\newcommand{\Iint}[2]
{\comp{\iint}{#1}{#2}}
\newcommand{\Int}[2]
% {\int\displaylimits_{#1}^{#2}}
{\int_{#1}^{#2}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\vsspan}{span}

% For hyperreference
\usepackage[bookmarks=true]{hyperref}

\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=blue,      
    urlcolor=blue,
    citecolor=blue,
}

\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
\def\e{\epsilon}
\def\g{\gamma}
\def\k{\kappa}
\def\o{\omega}
\def\s{\sigma}
\def\z{\zeta}
\def\x{\textbf{x}}
\def\t{\theta}
\def\vs{\varsigma}
\def\ve{\varepsilon}

\def\D{\Delta}
\def\S{\Sigma}
\def\G{\Gamma}

\def\R{\mathbb{R}}
\def\N{\mathbb{N}}

\def\ll{\left}
\def\rr{\right}

% Defining the algebraic quantities of motion
\def\quat{\mathbf{q}}
\newcommand{\sca}[1]{\l[#1\r]_{w}}
\newcommand{\vect}[1]{\l[#1\r]_{v}}
\def\pos{p}
\def\vel{\mathbf{v}}
\def\accel{\mathbf{a}}

% Geometric commands
\newcommand{\sksym}[1]{\floor{#1}_{\times}}
\newcommand{\fr}[1]{\texttt{#1}}
\newcommand{\qmatL}[1]{\floor{#1}_\ell}
\newcommand{\qmatR}[1]{\floor{#1}_r}
\newcommand{\vbf}[1]{{\bm{\mathbf{#1}}}}
\def\brc{\mathbf{brc}}
\def\calE{\mathcal{E}}

%Defining special notations for the optimization
\def\resi{\bm{r}}
\def\Lift{\mathcal{L}}
% \def\Jcb{\vbf{J}}

% Defining the Riemannian Groups
\def\bias{\mathbf{b}}
\def\noise{\bm{\eta}}
\def\rot{R}
\def\tf{T}
\def\trans{\mathbf{t}}
\def\SO{\mathrm{SO(3)}}
\def\so{\mathfrak{so}(3)}
\def\SE{\mathrm{SE(3)}}
\def\Rtoq{\mathcal{Q}}
\def\qtoR{\mathcal{R}}
\def\Exp{\text{Exp}}
\def\Log{\text{Log}}
\def\Hrj{\mathcal{H}}
\def\Omg{{\bm\Omega}}

\def\Scov{\textbf{C}}
\def\Smean{\textbf{S}}
\def\doteq{\leftarrow}

% Numbers
\def\ident{\mathbf{I}}
\def\zero{\mathbf{0}}

% Shorthands
\def\Dt{ {\D t} }
\def\dt{ {\d t} }
% Abbreviation
\def\wrt{\text{w.r.t. }}

% Shorthands for preintegrations
\def\pia{{\vbf{\a}}}
\def\pib{{\vbf{\b}}}
\def\pig{{\vbf{\g}}}
\def\pith{{\vbf{\theta}}}

% Defining the special quantities
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}
\def\Z{\mathcal{Z}}
\def\U{\mathcal{U}}
\def\I{\mathcal{I}}
\def\V{\mathcal{V}}
\def\M{\mathcal{M}}
\def\L{\mathcal{L}}
\def\P{\mathcal{P}}
\def\F{\mathcal{F}}
\def\C{\mathcal{C}}
\def\K{\mathcal{K}}
\def\T{\mathcal{T}}
\def\E{\mathcal{E}}

\def\angvel{\bm{\omega}}
\def\accel{\mathbf{a}}
\def\grav{\mathbf{g}}
\def\eulvec{\bm{\phi}}

% For remarks
\newtheorem{remark}{Remark}
\newtheorem{propo}{Proposition}

% Defining commonly used frames
\def\fA{\fr{A}}
\def\fB{\fr{B}}
\def\fC{\fr{C}}
\def\fL{\fr{L}}
\def\fW{\fr{W}}
\def\fI{\fr{I}}

% Short hand for the state estimate
\def\Xhat{\hat{\X}}
% Short hand for the sliding window state
\def\That{\hat{\T}}

% Shorthand for features coefficients
\def\f{\vbf{f}}
\def\n{\vbf{n}}
\def\m{\vbf{m}}
\def\Fbrv{\breve{\F}}

% Vector from antenna to anchor
\def\dis{\vbf{d}}

% Shorthand for quaternion elements
\def\Q{\mathbb{Q}}
\def\q{\mathbb{q}}

% Shorthand for underline
\newcommand{\ul}[1]{\underline{#1}}
% Shorthand for boldfont
\newcommand{\tb}[1]{\textbf{#1}}

\newcommand{\highlight}[1]{{\color{blue} #1}}

% Quick ref to a section
\newcommand{\sref}[1]{Sec. \ref{#1}}
% Quick ref to a Table
\newcommand{\tref}[1]{Tab. \ref{#1}}
% Quick ref to a Figure
\newcommand{\fref}[1]{Fig. \ref{#1}}

% Residual
\def\res{\vbf{r}}
% Transform
\def\tf{\vbf{T}}
\def\rot{\vbf{R}}
\def\pos{\vbf{p}}

\def\Ibf{\vbf{I}}
\def\Abf{\vbf{A}}
\def\dbf{\vbf{d}}
\def\Pbf{\vbf{P}}
\def\Sbf{\vbf{S}}
